Flipper games for monadically stable graph classes

A class of graphs $\mathscr{C}$ is monadically stable if for any unary expansion $\widehat{\mathscr{C}}$ of $\mathscr{C}$, one cannot interpret, in first-order logic, arbitrarily long linear orders in graphs from $\widehat{\mathscr{C}}$. It is known that nowhere dense graph classes are monadically stable; these encompass most of the studied concepts of sparsity in graphs, including graph classes that exclude a fixed topological minor. On the other hand, monadic stability is a property expressed in purely model-theoretic terms and hence it is also suited for capturing structure in dense graphs. For several years, it has been suspected that one can create a structure theory for monadically stable graph classes that mirrors the theory of nowhere dense graph classes in the dense setting. In this work we provide a step in this direction by giving a characterization of monadic stability through the Flipper game: a game on a graph played by Flipper, who in each round can complement the edge relation between any pair of vertex subsets, and Connector, who in each round localizes the game to a ball of bounded radius. This is an analog of the Splitter game, which characterizes nowhere dense classes of graphs (Grohe, Kreutzer, and Siebertz, J.ACM'17). We give two different proofs of our main result. The first proof uses tools from model theory, and it exposes an additional property of monadically stable graph classes that is close in spirit to definability of types. Also, as a byproduct, we give an alternative proof of the recent result of Braunfeld and Laskowski (arXiv 2209.05120) that monadic stability for graph classes coincides with existential monadic stability. The second proof relies on the recently introduced notion of flip-wideness (Dreier, M\"ahlmann, Siebertz, and Toru\'nczyk, ICALP 2023) and provides an efficient algorithm to compute Flipper's moves in a winning strategy.

==> afg/afg_flipwrap.tex <==
\subsection{Playing Multiple Flips}
\niko{The below proof assumes a variant of the Flipper game where Localizer is allowed to choose an induced subgraph of an $r$-ball (instead of the entire $r$-ball).
It is obvious that this only benefits Localizer. The proof of $\flipstar$ works for this version aswell, so we can just use this version in the algorithmic section and comment on this, for example in the definition of a Localizer strategy.
}
\begin{theorem}
    For every class of graphs $\CC$ and radius $r$,
    if there exists an $\ell$-winning $k$-move radius-$r$ Flipper strategy $\stratflip$ with runtime $f(n)$ on $\CC$, then there also exists an $(k\cdot \ell)$-winning $1$-move radius-$r$ Flipper strategy $\stratflip'$ with runtime $\Oof_k(f(n))$ on $\CC$.
\end{theorem}
\begin{proof}
    Intuitively, our new strategy $\stratflip'$ will work by wrapping $\stratflip$, queuing and applying its flips one by one, and preserving its internal state.
    Without loss of generality, we will assume that $\stratflip$ always returns a (multi)set of exactly $k$ flips, which can be achieved by filling up the returned flips with additional no-operation flips $\flip F = (\varnothing, \varnothing)$.

    An internal state $(\II_i,Q_i)$ of $\stratflip'$ consists of an internal state of $\stratflip$ and a queue of atomic flips.
    For every graph $G\in\CC$, the initial internal state of $\stratflip'$ is the initial internal state of $\stratflip$ and an empty queue.
    Let $\stratcon'$ be an arbitrary radius-$r$ Localizer strategy.
    We compute 
    \[
        ((\II_{i+1},Q_{i+1}), \flip F) = \stratflip'((\II_i,Q_i), \stratcon'(G_i)) 
    \]
    as follows.
    If $Q_i$ is empty, we query $\stratflip$ with internal state $\II_i$ and connector move $\stratcon'(G_i)$ to obtain the new internal state $\II_{i+1}$ and a set $F$ of exactly $k$ flips.
    We pick $\flip F$ to be an arbitrary flip from $F$ and set $Q_{i+1}$ to be an arbitrary ordering of $F$ without $\flip F$.

    Otherwise $Q_i$ is non-empty,
    so we can take a flip $\flip F$ from the queue, leaving us with the queue~$Q_{i+1}$ containing one less element.
    We preserve the internal state $\II_{i+1} := \II_i$ of $\stratflip$.

    It is easy to see that $\stratflip'$ has the desired runtime. 
    Let us now show that $\stratflip'$ is $(k\cdot \ell)$-winning.
    \begin{claim}\label{claim:ex_con}
        For every radius-$r$ Localizer strategy $\stratcon'$ and graph $G\in\CC$ with
        \[
            \RR(\stratcon',\stratflip',G) 
            =
            \big(G_0', (\II'_0,Q_0)\big), 
            \big(G_1', (\II'_1,Q_1)\big), 
            \big(G_2', (\II'_2,Q_2)\big), 
            \ldots
        \]
        there exists a radius-$r$ Localizer strategy $\stratcon$ with
        \[
            \RR(\stratcon,\stratflip,G) 
            =
            (G_0, \II_0), 
            (G_1, \II_1), 
            (G_2, \II_2), 
            \ldots
        \]
        such that for every $i \in \N$, $G'_{i\cdot k}$ is an induced subgraph of $G_i$ and $\II'_{i\cdot k} = \II_i$.

    \end{claim}

    Before proving the claim, we show that it implies that $\stratflip'$ is $(k\cdot \ell)$-winning.
    Given an arbitrary Localizer strategy $\stratcon'$, we have that there exist a strategy $\stratcon$ such that $G'_{\ell \cdot k}$ from $\RR(\stratcon',\stratflip',G)$ is an induced subgraph of $G_\ell$ from $\RR(\stratcon,\stratflip,G)$.
    By assumption $\stratflip$ is $\ell$-winning and both $G_\ell$ and $G'_{\ell \cdot k}$ must be the single vertex graph as desired.
    It remains to prove the claim.

    \begin{claimproof}
        We prove the claim by induction on $i$.
        For $i=0$ we trivially have $G'_{i\cdot 0} = G_0 = G$ and by construction $\II'_{i\cdot 0} = \II_0$ holds, no matter how $\stratcon$ is chosen.

        Assume now the claim holds for $i \geq 0$.
        By induction, $G'_{i\cdot k}$ is an induced subgraph of $G_i$ and $\II'_{i\cdot k} = \II_i$.
        We choose $\stratcon(G_i) := \stratcon'(G'_{i\cdot k})$.
        As $\stratcon'(G'_{i\cdot k})$ is a radius-$r$ Localizer strategy, $\stratcon'(G'_{i\cdot k})$ is an induced subgraph of a radius-$r$ ball in $G'_{i\cdot k}$.
        As $G'_{i\cdot k}$ is an induced subgraph of $G_i$, in particular $\stratcon'(G'_{i\cdot k})$ is an induced subgraph of a radius-$r$ ball in $G_i$. 
        Therefore our definition of $\stratcon(G_i)$ is a valid radius-$r$ Localizer move.
        It remains to show that $\II'_{(i+1)\cdot k} = \II_{i+1}$ and that $G'_{(i+1)\cdot k}$ is an induced subgraph of $G_{i+1}$.
        To prove the former, note that $\II'_{(i+1)\cdot k}$ is equal to the internal state $\II'_{i\cdot k+1}$, that was preserved while processing the non-empty queues $Q_{i\cdot k+1}\supsetneq \dots \supsetneq Q_{(i+1) \cdot k - 1}$ one flip at a time.
        By construction, we have 
        \[
            (F, \II'_{i\cdot k+1}) = \stratflip(\stratcon'(G'_{i\cdot k}), \II'_{i\cdot k}).
        \]
        By definition we have $\stratcon(G_i) = \stratcon'(G'_{i\cdot k})$ and by induction $\II'_{i\cdot k} = \II_i$. 
        Consequently
        \[
            (F, \II'_{i\cdot k+1} = \II_{i+1}) = \stratflip(\stratcon'(G'_{i\cdot k}), \II'_{i\cdot k}) = \stratflip(\stratcon(G_i), \II_i),
        \]
        which proves $\II'_{i\cdot k+1} = \II_{i+1}$
        and shows that the computed set of flips $F$ is the same in both runs.
        To show that $G'_{(i+1)\cdot k}$ is an induced subgraph of $G_{i+1} = \stratcon(G_i) \oplus F$, notice that also $G'_{(i+1)\cdot k}$ is obtained from $\stratcon(G_i) = \stratcon'(G'_{i\cdot k})$ by performing the flips $F$ and additionally localizing (i.e.\ taking induced subgraphs) between the atomic flips. 
        As flipping and taking induced subgraphs commutes (see \Cref{obs:subgraph_flip}), we conclude that $G'_{(i+1)\cdot k}$ is an induced subgraph of $G_{i+1}$.

    \end{claimproof}
    The proof of the claim completes the proof of the lemma.

    % \begin{claim}
    %     For every radius-$r$ Localizer strategy $\stratcon'$ and graph $G\in\CC$ with
    %     \[
    %         \RR(\stratcon',\stratflip',G) 
    %         =
    %         \big(G'_0, (\II_0,S_0)\big), 
    %         \big(G'_1, (\II_1,S_1)\big), 
    %         \big(G'_2, (\II_2,S_2)\big), 
    %         \ldots
    %     \]
    %     there exists a radius-$r$ Localizer strategy $\stratcon$ such that for every $i \in \N$ we have
    %     $(G_{0\cdot k}, \II_{0 \cdot k}),\ldots, 
    %     (G_{i \cdot k}, \II_{i \cdot k})$
    %     is an $i+1$ element prefix of $\RR(\stratcon,\stratflip,G)$.
    % \end{claim}

    % \begin{claim}
    %     For every radius-$r$ Localizer strategy $\stratcon'$ and graph $G\in\CC$ with
    %     \[
    %         \RR(\stratcon',\stratflip',G) 
    %         =
    %         \big(G_0, (\II_0,S_0)\big), 
    %         \big(G_1, (\II_1,S_1)\big), 
    %         \big(G_2, (\II_2,S_2)\big), 
    %         \ldots
    %     \]
    %     there exists a radius-$r$ Localizer strategy $\stratcon$ with
    %     \[
    %     \RR(\stratcon,\stratflip,G) = (G_{0\cdot k}, \II_{0 \cdot k}),    
    %     (G_{1 \cdot k}, \II_{1 \cdot k}),
    %     (G_{2 \cdot k}, \II_{2 \cdot k}), \ldots
    %     \]
    % \end{claim}
    % \begin{claimproof}
    %     Let $F_i = \{\flip F_{i\cdot k},\ldots,\flip F_{(i+1)\cdot k}\}$ be the flip played by $\stratflip'$ between the $(i\cdot k)$th and $((i+1)\cdot k)$th round.
    %     We have that $G_{(i+1)\cdot k}$ is an induced subgraph of $G^\mathrm{loc}_{i\cdot k} \oplus F_i$.
    %     % We construct the strategy $\s$
    % \end{claimproof}


    % \begin{claimproof}
    %     We prove the claim by induction on $i$.
    %     For $i=0$, the base case holds trivially as $(G_{0\cdot k} = G, \II_{0\cdot k} = \II_0(\stratflip,G))$ is the first position in any Flipper run for $\stratflip$ on $G$, no matter which Localizer strategy $\stratcon$ is chosen.

    %     Assume now the claim holds for $i \geq 0$.
    %     By induction we have that 
    %     $(G_{0\cdot k}, \II_{0 \cdot k}),\ldots, 
    %     (G_{i \cdot k}, \II_{i \cdot k})$
    %     is an $i+1$ element prefix of $\RR(\stratcon,\stratflip,G)$ for some radius-$r$ Localizer strategy $\stratcon$.
    %     Let us now describe $\stratcon(G_{i\cdot k})$, that is, the $(i+1)$st move of $\stratcon$ in the run $\RR(\stratcon,\stratflip,G)$.
    %     We choose 
    %     \[
    %         \stratcon(G_{i\cdot k}) 
    %         = 
    %         \stratcon'(G_{i \cdot k})[V(G_{(i+1) \cdot k})]
    %         .
    %     \]
    %     As $\stratcon'(G_{i \cdot k})$ is the induced subgraph of an radius-$r$ ball in $G_{i\cdot k}$,
    %     the same holds for $\stratcon(G_{i\cdot k})$, and we conclude that $\stratcon(G_{i\cdot k})$ is a valid radius-$r$ Localizer move.
    %     The $(i+2)$nd position of $\RR(\stratcon,\stratflip,G)$ is 
    %     $(\stratcon(G_{i\cdot k}) \oplus F, \II)$ where $(F, \II) = \stratflip(\stratcon(G_{i\cdot k}), \II_{i\cdot k})$.

    %     % By construction, $G_{(i+1) \cdot k}$ is obtained from $G_{i \cdot k}$ by playing the set of $k$ flips $F$, which is computed by $\stratflip(\II_{i \cdot k},\stratcon'(G_{i \cdot k}))$, and localizing in between.
    %     % We choose $\stratcon(G_{i\cdot k}) = \stratcon'(G_{i \cdot k})[V(G_{(i+1) \cdot k})]$
    %     % We have that $G_{(i+1) \cdot k}$ is an induced subgraph of
    %     % $G^\mathrm{loc}_{i \cdot k} \oplus F$

    % \end{claimproof}
\end{proof}

==> afg/afg_predictability_new.tex <==
Let us now show how to algorithmically predict the flips produced by $\cfw_r^\CC$.

\begin{lemma}[Predictability of $\cfw_r^\CC$]\label{lem:cfw_predictability}
	For every monadically stable class $\CC$ and radius $r\in\N$ there exists an algorithm $\guessflips_r^\CC$ that takes as input an $n$-vertex graph $G\in\CC$ and a subset $Z\subseteq V(G)$ and computes in time $\Oof_{\CC,r}(n^2)$ a set of at most $\wflips{r}{\CC}$ flips $F^\star$ such that
	for every set $X\subseteq V(G)$ with $\cfw_r^\CC(G,X) = (Y,F)$ we have: if $|Z|\geq 5$ and $Z\subseteq Y$, then $F = F^\star$.
\end{lemma}

\begin{proof}
	We will assume that $Z = \{z_1,\ldots,z_5\}$ contains exactly five vertices.
	If $Z$ is larger, we drop excess vertices. If $Z$ is smaller, we can just return $F^\star := \varnothing$.

	Let us now argue that in our description of the algorithm, we can also assume that the input satisfies $Z\subseteq Y$ from some $X\subseteq V(G)$ such that $\cfw_r^\CC(G,X) = (Y,F)$.
	If this is not the case, then we only have to ensure the bounds on the runtime and number of returned flips.
	A priori we cannot efficiently test whether $Z\subseteq Y$. 
	However, if we have an algorithm $\mathsf{ALG}$ that, assuming $Z \subseteq Y$, runs in the required time and produces the desired flips, we can enforce the desired bounds for any input~$Z$ by simulating $\mathsf{ALG}$ for the allowed number of runtime steps.
	If $\mathsf{ALG}$ does not terminate in the required time or has computed more that $\wflips{r}{\CC}$ flips, then we stop the execution and return $F^\star := \varnothing$.
	Otherwise we return the flips computed by $\mathsf{ALG}$.

	\medskip\noindent
	Let $X \subseteq V(G)$ be a set satisfying
	$\cfw_r^\CC(G,X) = (Y,F)$ and $Z\subseteq Y$.
	We will show how to compute from $G$ and $Z$ the flips $F^\star$ satisfying $F = F^\star$.
	We describe the algorithm by induction on $r$.
	The description will follow the definition of $\cfw_r^\CC$ as in the proof of \Cref{lem:cfw_wideness}. 
	In particular we will use the same notation.
	For $r=0$ we set $F^\star := \emptyset$ and we are done as also $F = \emptyset$.
	
	Assume $r>0$ and the predictability property has been proved for $r-1$.
	We compute $F^\star_{r-1} := \guessflips^\CC_{r-1}(G,Z)$ in time $\Oof_{\CC,r-1}(n^2)$ and set $H^\star := G \oplus F^\star_{r-1}$.
	As $Z \subseteq Y$, in particular $Z\subseteq Y_{r-1}$ for $(Y_{r-1},F_{r-1}) = \cfw_{r-1}^\CC(G,X)$ and by induction $F_{r-1} = F^\star_{r-1}$ and consequently $H = H^\star$.
	
	If $z_1$ and $z_2$ are at distance greater than $r$ in $H^\star$, we return $F^\star := F^\star_{r-1}$.
	In this case we have that $Y \supseteq \{z_1,z_2\}$ is distance-$r$ independent in $H = H^\star$ and consequently $F = F_{r-1} = F^\star_{r-1} = F^\star$.

	Otherwise, the vertices of $Y$ have pairwise distance exactly $r$.
	By using a breadth-first search, we mark the five balls $\BB^\star$ of radius $r' = \lceil r/2\rceil-1$ centered at the vertices from $Z$. 
	We have that $\BB^\star \subseteq \BB$. 
	We use the $\mathsf{Partition}$ algorithm from \Cref{lem:five} with input $H^\star$ and $\BB^\star$ to calculate the partition $\Pi^\star$ of $V(H^\star) = V(G)$ in time $\Oof(n^2)$.
	By \Cref{lem:five} we have $\Pi^\star = \Pi_{\mathfrak B}$ for the canonical ball classifier $\mathfrak{B} = (\BB, \bar s)$.
	Let $\bar s^\star$ be the tuple containing the minimum element of each part in $\Pi^\star$. 
	Since $\mathfrak{B} = (\BB, \bar s)$ is canonical, we have $\bar s^\star = \bar s$ (up to reordering). 
	Now let $\{V^\star_1,\ldots,V^\star_k\}$ be the parts of $\Pi_\star$ such that $s^\star_i := \min V^\star_i$ is adjacent to all the balls in $\BB^\star$ for $i\in[k]$.
	Since $(\BB,\bar s^\star)$ is a ball classifier, each $s^\star_i\in \bar s^\star$ is adjacent to either all or none of the balls from $\BB$.
	We therefore have that $s^\star_i = s_i$ and $V^\star_i = V_i$ for all $i\in[k]$ (up to reordering).
	Based on $H^\star$, $\{V^\star_1,\ldots, V^\star_k\}$, $\{s^\star_1,\ldots, s^\star_k\}$ and $r$, we can now follow the instructions from \Cref{lem:cfw_wideness} (the odd and the even case)  to compute a set of flips $F'$ in time $\Oof_{\CC,r}(n^2)$, such that we have $F^\star := F^\star_{r-1} \triangle F' = F$.
\end{proof}

As previously discussed, predictability implies canonicity, therefore combining \Cref{lem:cfw_wideness} and \Cref{lem:cfw_predictability} proves \Cref{lem:canonic_fuqw}.

